Equivariant log-concavity of graph matchings

For any graph, we show that the graded permutation representation of the graph automorphism group given by matchings is strongly equivariantly log-concave. The proof gives a family of equivariant injections inspired by a combinatorial map of Kratthenthaler and reduces to the hard Lefschetz theorem.

==> old.tex <==


    
    
    % We say that two pairs of matchings $(M, M'), (N, N')$ in $\mathbf{M}_{\ell - 1, k+1}(G_i)$ are $H_i$-equivalent if they agree on $H_i$; that is,
    % \[
    % M \cap H_i = N \cap H_i \textrm{ and } M' \cap H_i = N' \cap H_i. 
    % \]
    % \begin{figure}[h]
    %     \centering
    %     \includegraphics{figures/equivalent-pairs.pdf}
    %     \caption{In this example, we take $\ell = k = 8$, and the graph shown is the graph $G_i$ in question. The subgraph $H_i$ consists of just the square. The edges in the $7$-matching are indicated in blue, and the edges in the $9$-matching are indicated in pink. These two pairs of matchings agree on $H_i$, and so they give an equivalent pair of matchings in $\mathbf{M}_{7, 9}(G_i)$.}
    %     \label{fig:equivalent-pairs}
    % \end{figure}
    The set of $H_i$-equivalence classes is a partition of $\mathbf{M}_{\ell-1, k+1}(G_i)$, denoted as $\mathbf{P}_{\ell-1, k+1}(G_i)$.
    Similarly we define $H_i$-equivalence on $\mathbf{M}_{\ell, k}(G_i)$ and obtain a partition $\mathbf{M}_{\ell, k}(G_i)$, denoted as $\mathbf{P}_{\ell, k}(G_i)$. 
    
    In addition, we have 
    \begin{equation}
    \label{eq:partition-size}
        |\mathbf{P}_{\ell-1, k+1}(G_i)| = |\mathbf{P}_{\ell, k}(G_i)| = 2^{c_i},
    \end{equation}
    where $c_i$ is the number of connected components of $H_i$. 
    
    For any part $P$ of $\mathbf{P}_{\ell -1, k+1}(G_i)$, we define the subspace 
    \[
    V_{\ell-1, k+1}(P) := \Span\{x_{M} \otimes x_{M'} \colon (M, M') \in P\} \subseteq V_{\ell-1} \otimes V_{k+1}. 
    \]
    Similarly, for any part $P' \in \mathbf{P}_{\ell, k}(G_i)$, we define the subspace 
    \[
    V_{\ell, k}(P') := \Span\{x_{M} \otimes x_{M'} \colon (M, M') \in P'\} \subseteq V_{\ell} \otimes V_{k}.  
    \]
    Now, the vector space $V_{\ell-1} \otimes V_{k+1}$ admits the following direct sum decomposition 
    \begin{equation*}
        V_{\ell - 1} \otimes V_{k + 1} = \bigoplus_{G_i} \bigoplus_{P \in \mathbf{P}_{\ell-1, k+ 1}(G_i)} V_{\ell-1, k+1}(P). 
    \end{equation*}
    Similarly, the vector space $V_{\ell} \otimes V_{k}$ admits the following direct sum decomposition 
    \begin{equation*}
        V_{\ell} \otimes V_{k} = \bigoplus_{G_i} \bigoplus_{P \in \mathbf{P}_{\ell, k}(G_i)} V_{\ell, k}(P). 
    \end{equation*} In both decompositions, the graph $G_i$ ranges over all subgraphs of $G$ with $\ell + k$ edges. 
    
    We make the following observations. 
    First, for any $G_i$ and any part $P \in \mathbf{P}_{\ell - 1, k+1}(G_i)$, 
    the set 
    \[
    \bigcup_{(M, M') \in P} \N(M, M') 
    \] is a part of $\mathbf{P}_{\ell, k}(G_i)$. 
    Therefore, this set map 
    \[\mathbf{P}_{\ell - 1, k+1}(G_i) \to \mathbf{P}_{\ell, k}(G_i)\] given by sending every part $P$ in $\mathbf{P}_{\ell - 1, k+1}(G_i)$ to the union of all new matchings generated by pairs in $P$ as above is well-defined and injective. Combined with \cref{eq:partition-size}, this map is bijective. 

    Second, by definition of $\Phi_{\ell, k}$, we have that
    \[
    \Phi_{\ell, k}(V_{\ell-1, k+1}(P)) = V_{\ell, k}\left(\bigcup_{(M, M') \in P} \N(M, M') \right). 
    \]
    Since $\Phi_{\ell, k}$ restricted on $V_{\ell - 1, k+1}(P)$ is precisely the map defined in \cref{lem:linear-injection}, \cref{lem:linear-injection} shows that $\Phi_{\ell, k}$ is injective on each direct summand, proving the theorem. 
